MuTox: Universal MUltilingual Audio-based TOXicity Dataset and Zero-shot Detector

Research in toxicity detection in natural language processing for the speech modality (audio-based) is quite limited, particularly for languages other than English. To address these limitations and lay the groundwork for truly multilingual audio-based toxicity detection, we introduce MuTox, the first highly multilingual audio-based dataset with toxicity labels. The dataset comprises 20,000 audio utterances for English and Spanish, and 4,000 for the other 19 languages. To demonstrate the quality of this dataset, we trained the MuTox audio-based toxicity classifier, which enables zero-shot toxicity detection across a wide range of languages. This classifier outperforms existing text-based trainable classifiers by more than 1% AUC, while expanding the language coverage more than tenfold. When compared to a wordlist-based classifier that covers a similar number of languages, MuTox improves precision and recall by approximately 2.5 times. This significant improvement underscores the potential of MuTox in advancing the field of audio-based toxicity detection.

==> 40lang.tex <==
\subsection{Annotation for 19 + X additional languages}
\label{sec:19lang}


\paragraph{Preliminary selection.}  Based on annotated data in English and Spanish (section \ref{sec:datasetengspa}), we devise new criteria to select 4k sentences across 19 extra languages which we consider high-priority (HP) for the context of this work and related previous projects \cite{communication2023seamlessm4tmassively}. The purpose of this extension is to form a highly multilingual benchmark for audio-based toxicity classification. 

\textit{Languages}. Bengali, Dutch, French, German, Hindi, Indonesian, Italian, Japanese, Korean, Mandarin Chinese, Modern Standard Arabic, Portuguese, Russian, Swahili, Tagalog, Thai, Turkish, Urdu, Vietnamese.

\textit{Classifiers}. We use a text toxicity classifier that covers all these languages (\etox) in combination with the English toxicity classifier used in section \ref{sec:datasetengspa} (\detoxify). 

\textit{Datasets}. We use \speechmined{} which has parallel data \engx for all languages of interest.

\textit{Methodology}. We aim at finding 2,500 sentences with the n-largest toxicity scores, and randomly sample the dataset to complete the 4k set. Motivated by results from section \ref{sec:datasetengspa}, sentences are selected as follows:

We include all the samples positive per \etox and \detoxify scores higher than 0.8. This results in a small number of samples, ranging from 502 (deu) to less than 10 (hin, tgl, cmn)
Then, we include \etox detections (ignoring the \detoxify threshold) but allow only for a maximum of 200 sentences for each \etox token and add a maximum of 1,000 \etox sentences. We set these maxima so as to ensure toxicity diversity in the selection.
Finally, we include samples detected with \detoxify:
We use \detoxify in Italian, Portuguese, Turkish, Russian and French (which are supported by the tool). For the rest of non-supported languages, we resort to English \detoxify in the parallel text. [This method is supported as follows: on the corpus from section \ref{sec:datasetengspa}, we have a total toxicity of 0.25 in Spanish when using \detoxify in English with a threshold of 0.8].


\begin{figure}[ht!]
\center
    \includegraphics[width=7.5cm]{figures/19selection.png}
    \caption{Toxicity selection distribution per language (x-axis) and for each method: \detoxify, \etox and their intersection. }
    \label{fig:19selection}
\end{figure}

\paragraph{Dataset statistics and splits.} Figure \ref{fig:19selection} shows the results of this selection,  grouped by the methodology used (1 - intersection, 2 - \etox, 3 - \detoxify). Table \ref{tab:datasetspeech} shows the dataset splits. Our final dataset includes 120 hours.



==> datacard.tex <==
\label{app:datacard}
\newpage
\onecolumn
\begin{singlespace}
\tcbset{colback=white!10!white}
\begin{tcolorbox}[title=\textbf{\section{Data Card - MuTox}}]

%Dataset Description\footnote{We use a template for this data card {https://huggingface.co/docs/datasets/v1.12.0/dataset_card.html} 

Dataset Summary\footnote{We use a template for this data card {https://huggingface.co/docs/datasets/v1.12.0/dataset$\_$card.html}} 

\begin{itemize}
    \item \textit{MuTox is a speech and text dataset on 30 languages with toxicity labels.}
\end{itemize}

%\todo{Next table 1 summarizes the languages, source, total number of sentences and domains translated.}

How to use the data
\begin{itemize}
    \item \textit{You can access links to the data in the README at \url{https://github.com/facebookresearch/seamless_communication/tree/main/docs/rai/mutox_README.md}}
\end{itemize}

{Data Structure}
\begin{itemize}
    \item Languages: \textit{This version of MuTox cover a total of 35 languages see Table \ref{table:language_list} in Appendix \ref{app:lang}} 
\item Fields available: \textit{Speech source, Text source, Toxicity labels}
\end{itemize}

{Dataset Splits}
\begin{itemize}
    \item \textit{We provide training, dev, devtest and test splits as defined in Table \ref{tab:datasetspeech}}.
\end{itemize}

{Dataset Creation}
\begin{itemize}
\item Preprocessing steps: \textit{On speech,  we pre-filter audios by length between 2 and 8 seconds for convenience. On text, we pre-selected data based on all criteria described in section \ref{sec:guidelines}.}
\item Annotations \textit{Toxicity labels where produced based on annotation guidelines from section \ref{sec:guidelines}. }
\item Personal and Sensitive Information: \textit{Not applicable}
\end{itemize}


{Considerations for Using the Data}
 %  \item Details on the dataset(s) used for the quantitative analyses in the card. \\
\begin{itemize}
    \item Social Impact of Dataset: \textit{The dataset is built to increase toxicity detection quality in speech and text natural language applications.} 
%\item Discussion of Biases \marta{todo, run the GenderGAP pipeline}
\end{itemize}

{Additional Information}
\begin{itemize}
\item Licensing Information \textit{We are releasing training, dev and devtest splits under the terms of MIT License%\footnote{https://www.creativecommons.org/licenses/by-nc/4.0/}
}
\item Citation Information\\
\textit{Marta R. Costa-jussà, Mariano Coria Meglioli, Pierre Andrews,
David Dale, Prangthip Hansanti, Elahe Kalbassi,
Alex Mourachko, Christophe Ropers, Carleigh Wood},  MuTox: Universal MUltilingual Audio-based TOXicity Dataset and Zero-shot Detector, arxiv, 2024

\end{itemize}

\end{tcolorbox}
\end{singlespace}


==> modelcard.tex <==
\newpage
\onecolumn
\label{app:modelcard}
%\begin{adjustwidth}{-5pt}{-2pt}
\begin{singlespace}
\tcbset{colback=white!10!white}
\begin{tcolorbox}[title=\textbf{\section{Model Card - MuTox}}]

Model Details% \footnote{For this card, we use the template from \cite{10.1145/3287560.3287596}.  

   
\begin{itemize}
\setlength\itemsep{0.0001em}
\item Person or organization developing model: \textit{Developed by FAIR at Meta}
\item Model date: \textit{November 30, 2023}
%\item Model version: 
%\item Model type: 
\item License: \textit{CC-BY-NC 4.0}
%\footnote{\url{https://creativecommons.org/licenses/by-nc/4.0/legalcode}}}
%\item Where to send questions or comments about the model: \url{https://github.com/facebookresearch/stopes/issues}
\end{itemize}

Intended Use
\begin{itemize}
\setlength\itemsep{0.0001em}
    \item Primary intended uses: \textit{Automatic detection of toxicity for speech and text.}
\item Information on how to use the model can be found in the Seamless$\_$communication repository: \url{https://github.com/facebookresearch/seamless_communication/tree/main/src/seamless_communication/toxicity}
\item Primary intended users: \textit{Primary users are researchers and speech translation research community. }
%\item Out-of-scope use cases: \textit{}
\end{itemize}


{Metrics}
\begin{itemize}
  \item Model performance measures: \textit{AUC, Precision and Recall}
\end{itemize}

{Data}
\begin{itemize}
\item Training and Evaluation data: \textit{Detoxy \cite{Ghosh2021DeToxyAL}, JigSaw \cite{jigsaw-dataset} and MuTox Corpus}, see Table \ref{tab:datasetspeech} and MuTox data card in appendix \ref{app:datacard}.
\end{itemize}

{Ethical Considerations}
\begin{itemize}
 \item \textit{The training data used for model development were mined from various publicly available sources on the web. Although we invested heavily in data cleaning, personally identifiable
 information may not be entirely eliminated. However, as the model is not generative, it is unlikely that such information could be recovered from the model.
} 
\item \textit{We did not specifically study possible biases of the model.} 
\end{itemize}

%\begin{mcsection}
Caveats and Recommendations
\begin{itemize}
  \item{Limitations: \textit{Researchers should consider extending data to other languages and more types of toxicity when using the model in a research application.}}
  \end{itemize}

Citation Information\\
\textit{Marta R. Costa-jussà, Mariano Coria Meglioli, Pierre Andrews,
David Dale, Prangthip Hansanti, Elahe Kalbassi,
Alex Mourachko, Christophe Ropers, Carleigh Wood},  MuTox: Universal MUltilingual Audio-based TOXicity Dataset and Zero-shot Detector, arxiv, 2024
%\end{mcsection}

\end{tcolorbox}
\end{singlespace}
%\end{adjustwidth}

